Feature Extractor or Decision Maker: Rethinking the Role of Visual Encoders in Visuomotor Policies

An end-to-end (E2E) visuomotor policy is typically treated as a unified whole, but recent approaches using out-of-domain (OOD) data to pretrain the visual encoder have cleanly separated the visual encoder from the network, with the remainder referred to as the policy. We propose Visual Alignment Testing, an experimental framework designed to evaluate the validity of this functional separation. Our results indicate that in E2E-trained models, visual encoders actively contribute to decision-making resulting from motor data supervision, contradicting the assumed functional separation. In contrast, OOD-pretrained models, where encoders lack this capability, experience an average performance drop of 42\% in our benchmark results, compared to the state-of-the-art performance achieved by E2E policies. We believe this initial exploration of visual encoders' role can provide a first step towards guiding future pretraining methods to address their decision-making ability, such as developing task-conditioned or context-aware encoders.

==> body/discussion.tex <==
In \textit{Fig.}~\ref{fig:saliency_3}, we demonstrate that the decision-making ability of E2E encoders extends to multi-task settings, where they differentiate between tasks and focus on task-relevant features accordingly.
This alleviates concerns that their decision-making ability results from overfitting to a single task.
Furthermore, \textit{Fig.}~\ref{fig:saliency_1} shows that ImageNet features effectively recognize large objects in a scene, capturing most key information. This non-specific yet information-rich property likely explains ImageNet's superior performance compared to other pretrained encoders.
For completeness, \textit{Tab.}~\ref{tab:finetune} shows that finetuning pretrained encoders can enhance their performance, which does not contradict our conclusions. Investigating optimal finetuning methods and how they influence the representations lies beyond the scope of this study.

==> pics/main_results_illustration.tex <==
\centering
\subfloat[\centering Out-of-domain pretrain]{{\includegraphics[width=0.46\textwidth]{pics/fig2/in_domain.png} }}%
\qquad
\subfloat[\centering Task-aware pretrain]{{\includegraphics[width=0.46\textwidth]{pics/fig2/task_aware_2.png} }}%


==> pics/saliency_task_aware.tex <==
\minipage{0.32\textwidth}
    \includegraphics[width=\linewidth]{pics/saliency/spam.png}
\endminipage\hfill
\minipage{0.32\textwidth}
    \includegraphics[width=\linewidth]{pics/saliency/square.png}
\endminipage\hfill
\minipage{0.32\textwidth}%
    \includegraphics[width=\linewidth]{pics/saliency/can.png}
\endminipage

==> tables/discussion_main.tex <==
% \centering
% \subfloat[\centering Success rates for in-domain pretraining. Training is conducted for 300 epochs.]{\input{tables/exp_indomain_avg}}%
% \qquad
% \subfloat[\centering Success rates for fine-tuning. All models are trained with DP-C as downstream policy.]{\input{tables/exp_transfer/transfer_finetune}}%

==> tables/exp_baseline/bl_can.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{Pre-training} &  \\
\toprule
 & ImageNet & R3M & MVP & VIP & E2E \\
\midrule
BC & nan & 0.58 & 0.48 & 0.2 & 0.9 \\
BC-RNN & nan & nan & nan & nan & 0.86 \\
DP-CNN & 1.0 & 0.96 & nan & 0.44 & 1.0 \\
DP-Trans & 1.0 & 0.92 & nan & 0.6 & 0.96 \\
\bottomrule
\end{tabular}
\caption{can}
\label{tab:your_label}


==> tables/exp_baseline/bl_nut_ass.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{Pre-training} &  \\
\toprule
 & ImageNet & R3M & MVP & VIP & E2E \\
\midrule
BC & nan & nan & 0.0 & 0.0 & nan \\
BC-RNN & 0.09 & 0.03 & nan & nan & 0.2 \\
DP-CNN & nan & 0.08 & 0.16 & 0.0 & nan \\
DP-Trans & nan & 0.06 & 0.04 & 0.02 & 0.14 \\
\bottomrule
\end{tabular}
\caption{nut\_ass}
\label{tab:your_label}



==> tables/exp_baseline/bl_pusht.tex <==
\centering
\begin{tabular}{ccccc|c}
% \toprule
Policy & \multicolumn{4}{c}{Pre-training} &  \\
\toprule
 & ImageNet & R3M & MVP & VIP & E2E \\
\midrule
BC & 0.15 & 0.236 & 0.122 & 0.116 & 0.657 \\
% \midrule
BC-RNN & 0.337 & 0.489 & nan & 0.125 & 0.657 \\
% \midrule
DP-CNN & nan & 0.679 & 0.776 & 0.263 & 0.938 \\
% \midrule
DP-Trans & nan & 0.673 & 0.682 & 0.269 & nan \\
\bottomrule
\end{tabular}
\caption{pusht}
\label{tab:pusht}

==> tables/exp_baseline/bl_square.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{Pre-training} &  \\
\toprule
 & ImageNet & R3M & MVP & VIP & E2E \\
\midrule
BC & nan & 0.2 & 0.12 & nan & 0.52 \\
BC-RNN & 0.6 & nan & nan & nan & 0.76 \\
DP-CNN & nan & 0.52 & nan & 0.06 & 0.92 \\
DP-Trans & 0.74 & 0.5 & nan & 0.16 & 0.88 \\
\bottomrule
\end{tabular}
\caption{square}
\label{tab:your_label}


==> tables/exp_baseline/bl_stack.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{Pre-training} &  \\
\toprule
 & ImageNet & R3M & MVP & VIP & E2E \\
\midrule
BC & nan & 0.36 & 0.34 & 0.02 & 0.8 \\
BC-RNN & 0.62 & 0.66 & nan & nan & 0.92 \\
DP-CNN & 0.76 & 0.78 & nan & 0.04 & 1.0 \\
DP-Trans & 0.86 & 0.72 & nan & 0.2 & 0.92 \\
\bottomrule
\end{tabular}
\caption{stack}
\label{tab:your_label}


==> tables/exp_baseline/bl_stack_three.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{Pre-training} &  \\
\toprule
 & ImageNet & R3M & MVP & VIP & E2E \\
\midrule
BC & nan & nan & 0.0 & 0.0 & nan \\
BC-RNN & 0.02 & 0.0 & nan & nan & 0.1 \\
DP-CNN & nan & 0.02 & 0.02 & 0.0 & nan \\
DP-Trans & 0.0 & 0.02 & 0.0 & 0.0 & nan \\
\bottomrule
\end{tabular}
\caption{stack\_three}
\label{tab:your_label}


==> tables/exp_in_domain/in_domain_can.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{In-domain Pre-training} &  \\
\toprule
 & BC & BC-RNN & DP-CNN & DP-Trans & E2E \\
\midrule
BC & -- & \textbf{0.94} & 0.84 & 0.88 & 0.90 \\
BC-RNN & 0.92 & -- & 0.98 & \underline{\textbf{1.00}} & 0.98 \\
DP-CNN & 0.96 & 0.96 & -- & 0.96 & \underline{\textbf{1.00}} \\
DP-Trans & 0.82 & 0.90 & \textbf{0.98} & -- & 0.96 \\
\bottomrule
\end{tabular}
% \caption{can}
\label{tab:your_label}


==> tables/exp_in_domain/in_domain_main.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{In-domain Pre-training} &  \\
\toprule
 & BC & BC-RNN & DP-CNN & DP-Trans & E2E \\
\midrule
BC & -- & -- & 0.84 & 0.88 & 0.90 \\
BC-RNN & -- & -- & -- & -- & 0.98 \\
DP-CNN & 0.96 & -- & -- & 0.96 & 1.00 \\
DP-Trans & 0.82 & -- & 0.98 & -- & 0.96 \\
\bottomrule
\end{tabular}
\caption{can}
\label{tab:your_label}

==> tables/exp_in_domain/in_domain_pusht.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{In-domain Pre-training} &  \\
\toprule
 & BC & BC-RNN & DP-CNN & DP-Trans & E2E \\
\midrule
BC & -- & 0.48 & 0.30 & \textbf{0.68} & 0.66 \\
BC-RNN & 0.76 & -- & 0.83 & \textbf{0.88} & 0.76 \\
DP-CNN & 0.84 & 0.80 & -- & 0.88 & \underline{\textbf{0.94}} \\
DP-Trans & 0.64 & 0.78 & 0.80 & -- & \textbf{0.91} \\
\bottomrule
\end{tabular}
% \caption{pusht}
\label{tab:your_label}


==> tables/exp_in_domain/in_domain_square.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{In-domain Pre-training} &  \\
\toprule
 & BC & BC-RNN & DP-CNN & DP-Trans & E2E \\
\midrule
BC & -- & 0.26 & \textbf{0.60} & 0.52 & 0.52 \\
BC-RNN & 0.58 & -- & \textbf{0.88} & 0.86 & 0.74 \\
DP-CNN & 0.62 & 0.66 & -- & 0.88 & \textbf{0.92} \\
DP-Trans & 0.36 & 0.58 & \underline{\textbf{0.94}} & -- & 0.88 \\
\bottomrule
\end{tabular}
% \caption{square}
\label{tab:your_label}


==> tables/exp_in_domain/in_domain_stack.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{In-domain Pre-training} &  \\
\toprule
 & BC & BC-RNN & DP-CNN & DP-Trans & E2E \\
\midrule
BC & -- & \textbf{0.80} & 0.62 & 0.74 & \textbf{0.80} \\
BC-RNN & 0.90 & -- & 0.92 & 0.86 & \textbf{0.96} \\
DP-CNN & 0.90 & 0.90 & -- & 0.96 & \underline{\textbf{1.00}} \\
DP-Trans & 0.92 & \textbf{0.94} & 0.80 & -- & 0.92 \\
\bottomrule
\end{tabular}
% \caption{stack}
\label{tab:your_label}


==> tables/exp_in_domain_best_3/can.tex <==
\centering
\begin{tabular}{ccccc|c}
    Policy & \multicolumn{4}{c}{In-domain Pre-training} &  \\
    \toprule
     & BC & BC-RNN & DP-CNN & DP-Trans & E2E \\
    \midrule
    BC & -- & \textbf{0.92} & 0.78 & 0.86 & 0.89 \\
    BC-RNN & 0.90 & -- & 0.97 & \textbf{0.98} & \textbf{0.98} \\
    DP-CNN & 0.95 & 0.95 & -- & 0.96 & \textbf{1.00} \\
    DP-Trans & 0.82 & 0.87 & 0.95 & -- & \textbf{0.96 }\\
    \bottomrule
\end{tabular}
\label{tab:your_label}


==> tables/exp_in_domain_best_3/pusht.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{In-domain Pre-training} &  \\
\toprule
 & BC & BC-RNN & DP-CNN & DP-Trans & E2E \\
\midrule
BC & -- & 0.47 & 0.30 & \textbf{0.67} & 0.64 \\
BC-RNN & 0.74 & -- & 0.78 & \textbf{0.88} & 0.74 \\
DP-CNN & 0.82 & 0.79 & -- & 0.86 & \textbf{0.93} \\
DP-Trans & 0.63 & 0.77 & 0.79 & -- & \textbf{0.89} \\
\bottomrule
\end{tabular}
\label{tab:your_label}


==> tables/exp_in_domain_best_3/square.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{In-domain Pre-training} &  \\
\toprule
 & BC & BC-RNN & DP-CNN & DP-Trans & E2E \\
\midrule
BC & -- & 0.25 & 0.51 & 0.51 & \textbf{0.52} \\
BC-RNN & 0.56 & -- & \textbf{0.86} & 0.84 & 0.69 \\
DP-CNN & 0.61 & 0.65 & -- & 0.86 & \textbf{0.91} \\
DP-Trans & 0.33 & 0.56 & 0.86 & -- & \textbf{0.87} \\
\bottomrule
\end{tabular}
\label{tab:your_label}


==> tables/exp_in_domain_best_3/stack.tex <==
\centering
\begin{tabular}{ccccc|c}
Policy & \multicolumn{4}{c}{In-domain Pre-training} &  \\
\toprule
 & BC & BC-RNN & DP-CNN & DP-Trans & E2E \\
\midrule
BC & -- & 0.77 & 0.61 & 0.68 & \textbf{0.78} \\
BC-RNN & 0.88 & -- & 0.92 & 0.84 & \textbf{0.96} \\
DP-CNN & 0.89 & 0.89 & -- & 0.93 & \textbf{0.97} \\
DP-Trans & 0.83 & 0.89 & 0.80 & -- & \textbf{0.91} \\
\bottomrule
\end{tabular}
\label{tab:your_label}


==> tables/exp_in_domain_pure_number/can.tex <==
 BC & -- & \textbf{0.92} & 0.78 & 0.86 & 0.89 \\
 BC-RNN & 0.90 & -- & 0.97 & \textbf{0.98} & \textbf{0.98} \\
 DP-CNN & 0.95 & 0.95 & -- & 0.96 & \textbf{1.00} \\
 DP-Trans & 0.82 & 0.87 & 0.95 & -- & \textbf{0.96 }

==> tables/exp_in_domain_pure_number/pusht.tex <==
BC & -- & 0.47 & 0.30 & \textbf{0.67} & 0.64 \\
 BC-RNN & 0.74 & -- & 0.78 & \textbf{0.88} & 0.74 \\
 DP-CNN & 0.82 & 0.79 & -- & 0.86 & \textbf{0.93} \\
 DP-Trans & 0.63 & 0.77 & 0.79 & -- & \textbf{0.89} 

==> tables/exp_in_domain_pure_number/square.tex <==
BC & -- & 0.25 & 0.51 & 0.51 & \textbf{0.52} \\
BC-RNN & 0.56 & -- & \textbf{0.86} & 0.84 & 0.69 \\
DP-CNN & 0.61 & 0.65 & -- & 0.86 & \textbf{0.91} \\
DP-Trans & 0.33 & 0.56 & 0.86 & -- & \textbf{0.87}

==> tables/exp_in_domain_pure_number/stack.tex <==
BC & -- & 0.77 & 0.61 & 0.68 & \textbf{0.78} \\
BC-RNN & 0.88 & -- & 0.92 & 0.84 & \textbf{0.96} \\
DP-CNN & 0.89 & 0.89 & -- & 0.93 & \textbf{0.97} \\
DP-Trans & 0.83 & 0.89 & 0.80 & -- & \textbf{0.91}

==> tables/exp_indomain_avg.tex <==
% \begin{tabular}{lccccc}
%      \toprule
%      \textbf{Policy} & \multicolumn{4}{c}{\textbf{In-domain}} & \textbf{E2E}\\
%      \cmidrule(lr){2-5}
%      & BC & BC-RNN & DP-C & DP-T & \\
%      \toprule
%      BC & -- & 0.60 & 0.55 & \underline{0.68} & \textbf{0.71} \\
%      BC-RNN & 0.77 & -- & \underline{0.88} & \textbf{0.89} & 0.84 \\
%      DP-C & 0.82 & 0.82 & -- & \underline{0.90} & \textbf{0.95} \\
%      DP-T & 0.65 & 0.77 & \underline{0.85} & -- & \textbf{0.91} \\
%      \bottomrule
% \end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\scalebox{0.78}{
\begin{tabular}{lccccc}
     &\multicolumn{4}{c}{\textbf{In-domain}}&\\
     \toprule
     \textbf{Policy} & BC & BC-RNN & DP-C & DP-T & \textbf{E2E}\\
     \toprule
     BC & -- & 0.60 & 0.55 & \underline{0.68} & \textbf{0.71} \\
     BC-RNN & 0.77 & -- & \underline{0.88} & \textbf{0.89} & 0.84 \\
     DP-C & 0.82 & 0.82 & -- & \underline{0.90} & \textbf{0.95} \\
     DP-T & 0.65 & 0.77 & \underline{0.85} & -- & \textbf{0.91} \\
     \bottomrule
\end{tabular}
}

==> tables/exp_task_aware.tex <==
\centering
\subfloat[\centering Success rates in \textcolor{brown}{simulation} and \textcolor{lime}{real-world}.]{\input{tables/exp_transfer/transfer}}%
\qquad
\subfloat[\centering Evaluation loss for UR5 Reach task.]{\includegraphics[width=0.5\linewidth]{pics/exps/spam_mug_full.png}}%

==> tables/exp_transfer/transfer_finetune.tex <==
% \centering
% \begin{tabular}{ccccccccc|c}
%     \toprule
%     Tasks  & BC & BC\_RNN & DP\_CNN & DP\_Trans \\
%     \midrule
%     Pick Place  &  0.28 & 0.20 & 0.28 & 0.24 \\
%     % Stack Three & 0.47 & 0.61 & 0.63 & 0.51 \\
%     Nut Assembly & 0.49 & 0.43 & 0.55 & 0.54 \\
%     \bottomrule
% \end{tabular}
% \caption{Transfer Finetune}
% \label{tab:your_label}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \centering
% \begin{tabular}{lcccccccccc}
%     \toprule
%     \textbf{Task} & \multicolumn{3}{c}{\textbf{Out-of-domain}} & \multicolumn{4}{c}{\textbf{In-domain}} & \textbf{E2E} \\
%     \cmidrule(lr){2-4} \cmidrule(lr){5-8}
%      & \text{Imagenet} & \text{R3M} & \text{MVP} & \text{BC} & \text{BC\_RNN} & \text{ DP\_CNN} & \text{ DP\_Trans}\\
%     \midrule
%     Pick Place  & 0.00 & 0.00 & 0.04 & 0.28 & 0.20 & 0.28 & 0.24 & \textbf{0.36}\\
%     Stack Three &  0.00 & 0.00 & 0.05 & 0.47 & 0.61 & \textbf{0.63} & 0.51 & 0.60\\
%     Nut Assembly & 0.00 & 0.00 & 0.11 & 0.49 & 0.43 & \textbf{0.55} & 0.54 & 0.54\\
%     \bottomrule
% \end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lcccccccccc}
%     \toprule
%     \textbf{Task} & \multicolumn{3}{c}{\textbf{Out-of-domain}} & \multicolumn{4}{c}{\textbf{In-domain}} & \textbf{E2E} \\
%     \cmidrule(lr){2-4} \cmidrule(lr){5-8}
%      & \text{Imagenet} & \text{R3M} & \text{MVP} & \text{BC} & \text{BC\_RNN} & \text{ DP\_CNN} & \text{ DP\_Trans}\\
%     \midrule
%     Pick Place  & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.04\textcolor{green}{$\downarrow_{43\%}$} & 0.28\textcolor{red}{$\uparrow_{300\%}$} & 0.20\textcolor{red}{$\uparrow_{233\%}$} & 0.28\textcolor{red}{$\uparrow_{367\%}$} & 0.24\textcolor{red}{$\uparrow_{243\%}$} & \textbf{0.36}\\
%     Stack Three &  0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.05\textcolor{green}{$\downarrow_{0\%}$} & 0.47\textcolor{red}{$\uparrow_{840\%}$} & 0.61\textcolor{red}{$\uparrow_{239\%}$} & \textbf{0.63}\textcolor{red}{$\uparrow_{250\%}$} & 0.51\textcolor{red}{$\uparrow_{750\%}$} & 0.60\\
%     Nut Assembly & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.11\textcolor{green}{$\downarrow_{35\%}$} & 0.49\textcolor{red}{$\uparrow_{104\%}$} & 0.43\textcolor{red}{$\uparrow_{54\%}$} & \textbf{0.55}\textcolor{red}{$\uparrow_{28\%}$} & 0.54\textcolor{red}{$\uparrow_{0\%}$} & 0.54\\
%     \bottomrule
% \end{tabular}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \centering
% \begin{tabular}{lccccccc}
%     \toprule
%     \textbf{Task} & \multicolumn{3}{c}{\textbf{Out-of-domain}} & \multicolumn{1}{c}{\textbf{In-domain}} & \textbf{E2E} \\
%     \cmidrule(lr){2-4}
%      & \text{Imagenet} & \text{R3M} & \text{MVP} & &\\
%     \midrule
%     \textit{Pick Place} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.04\textcolor{green}{$\downarrow_{43\%}$} & 0.28\textcolor{red}{$\uparrow_{367\%}$} & \textbf{0.36}\\
%     \textit{Stack Three} &  0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.05\textcolor{green}{$\downarrow_{0\%}$} & \textbf{0.63}\textcolor{red}{$\uparrow_{250\%}$} & 0.60\\
%     \textit{Nut Assembly} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.11\textcolor{green}{$\downarrow_{35\%}$} & \textbf{0.55}\textcolor{red}{$\uparrow_{28\%}$} & 0.54\\
%     \bottomrule
% \end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \centering
% \begin{tabular}{lcccc}
%     \toprule
%     \textbf{Task} & \multicolumn{3}{c}{\textbf{Out-of-domain}} & \textbf{E2E} \\
%     \cmidrule(lr){2-4}
%      & \text{ImageNet} & \text{R3M} & \text{MVP} &\\
%     \toprule
%     \textit{Pick Place} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.04\textcolor{green}{$\downarrow_{43\%}$} & \textbf{0.36}\\
%     % \textit{Stack Three} &  0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.05\textcolor{green}{$\downarrow_{0\%}$} & 0.60\\
%     \textit{Nut Assembly} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.11\textcolor{green}{$\downarrow_{35\%}$} & \textbf{0.54}\\
%     \bottomrule
% \end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\scalebox{0.72}{
\centering
\begin{tabular}{lcccc}
    &\multicolumn{3}{c}{\textbf{Out-of-domain}}&\\
    \toprule
    \textbf{Task} & \text{ImageNet} & \text{R3M} & \text{MVP} & \textbf{E2E} \\
    \toprule
    \textit{Pick Place} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & \underline{0.04}\textcolor{green}{$\downarrow_{43\%}$} & \textbf{0.36}\\
    \textit{Nut Assembly} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & 0.00\textcolor{green}{$\downarrow_{100\%}$} & \underline{0.11}\textcolor{green}{$\downarrow_{35\%}$} & \textbf{0.54}\\
    \bottomrule
\end{tabular}
}
